Room impulse response reconstruction with physics-informed deep learning

A method is presented for estimating and reconstructing the sound field within a room using physics-informed neural networks. By incorporating a limited set of experimental room impulse responses as training data, this approach combines neural network processing capabilities with the underlying physics of sound propagation, as articulated by the wave equation. The network's ability to estimate particle velocity and intensity, in addition to sound pressure, demonstrates its capacity to represent the flow of acoustic energy and completely characterise the sound field with only a few measurements. Additionally, an investigation into the potential of this network as a tool for improving acoustic simulations is conducted. This is due to its profficiency in offering grid-free sound field mappings with minimal inference time. Furthermore, a study is carried out which encompasses comparative analyses against current approaches for sound field reconstruction. Specifically, the proposed approach is evaluated against both data-driven techniques and elementary wave-based regression methods. The results demonstrate that the physics-informed neural network stands out when reconstructing the early part of the room impulse response, while simultaneously allowing for complete sound field characterisation in the time domain.

==> Makefile <==
OUTPUT = ./publish
XELATEX=xelatex -file-line-error -interaction=nonstopmode

UNAME := $(shell uname)
ifeq ($(UNAME), Linux)
	DTUDIR = /home/manu
endif
ifeq ($(UNAME), Darwin)
	DTUDIR = /Users/mha/dtu
endif

all: publish # wip

.PHONY: publish draft-tex jasa figures bib beamer clean-post-build

beamer: pdf-figures
	xelatex beamer.tex
	#bibtex beamer.aux
	#xelatex beamer.tex
	#xelatex beamer.tex

bib: 
	@echo " > Collect bibliography..."
	@python3 $(DTUDIR)/l_bib/gen_bibliography.py bibliography.bib 1> /dev/null

wip: main.tex
	latexmk -pdf -pdflatex="$(XELATEX)" -use-make -pvc main.tex

wipt: main.tex bib
	latexmk -pdf -pdflatex="$(XELATEX)" main.tex -f

arxiv: #figures bib
	@echo " > Compile arxiv version..."
	@xelatex "\def\input{main.tex}" 1> /dev/null
	@xelatex "\def\input{main.tex}" 1> /dev/null
	@mv main.pdf arxiv.pdf

thesis: #figures bib
	@echo " > Compile thesis version..."
	@xelatex "\def\thesis{}\input{main.tex}" 1> /dev/null
	@xelatex "\def\thesis{}\input{main.tex}" 1> /dev/null
	@mv main.pdf hahmann2022csc.pdf

jasa: #figures bib
	@echo " > Compile manuscript version..."
	@xelatex "\def\manuscript{}\input{main.tex}" 1> /dev/null
	@xelatex "\def\manuscript{}\input{main.tex}" 1> /dev/null
	@mv main.pdf manuscript.pdf
	@echo " > Compile reviewer version..."
	@xelatex "\def\reviewers{}\input{main.tex}" 1> /dev/null
	@xelatex "\def\reviewers{}\input{main.tex}" 1> /dev/null
	@mv main.pdf reviewers.pdf
	@echo " > Compile reprint version..."
	@xelatex "\def\reprint{}\input{main.tex}" 1> /dev/null
	@xelatex "\def\reprint{}\input{main.tex}" 1> /dev/null
	@mv main.pdf reprint.pdf
	#@echo " > Compile letter to editor..."
	#@xelatex letter.tex
	@echo " > Convert reprint to greyscale..."
	@@gs \
		-sDEVICE=pdfwrite \
		-sProcessColorModel=DeviceGray \
		-sColorConversionStrategy=Gray \
		-dPDFUseOldCMS=false \
		-q \
		-o reprint_greyscale.pdf \
		-f reprint.pdf

rebuttal:
	@xelatex rebuttal_letter.tex 1> /dev/null

publish: jasa rebuttal
	@echo " > Publish files..."
	@mkdir -p $(OUTPUT)
	@touch $(OUTPUT)/dummy
	@rm $(OUTPUT)/*
	@cp main.tex              $(OUTPUT)/manuscript.tex
	@cp manuscript.pdf        $(OUTPUT)/manuscript.pdf
	@cp reprint.pdf           $(OUTPUT)/reprint.pdf
	@cp reprint_greyscale.pdf $(OUTPUT)/reprint_greyscale.pdf
	@cp reviewers.pdf         $(OUTPUT)/reviewers.pdf
	@cp rebuttal_letter.pdf   $(OUTPUT)/rebuttal_letter.pdf
	@cp ./fig/Figure*pdf $(OUTPUT)/

figures: #pdf-figures
	@echo " > Compile TeX figures..."
	make -C fig 1> /dev/null
	@cp "./fig/1dpartitioning.pdf"                        ./fig/Figure1.pdf
	@cp "./fig/rec_1dcsc.pdf"                             ./fig/Figure2.pdf
	@cp "./fig/nmse_distance_monopole.pdf"                ./fig/Figure3.pdf
	@cp "./fig/rec_monoplane_343_gpwe_lpwe_cpwe_cpwe.pdf" ./fig/Figure4.pdf
	@cp "./fig/vector_fields.pdf"                         ./fig/Figure5.pdf
	@cp "./fig/classroom.pdf"                             ./fig/Figure6.pdf
	@cp "./fig/rec_019_1000_gpwe_lpwe_cpwe_cpwe.pdf"      ./fig/Figure7.pdf
	@cp "./fig/csc_paper_xfreq_mic_nmse.pdf"              ./fig/Figure8.pdf

pdf-figures:
	@echo " > Copy pdf figures..."
	mkdir -p fig
	@cp $(DTUDIR)/rat/figures/reconstructions/rec_019_1000_gpwe_lpwe_cpwe_cpwe.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/reconstructions/rec_monoplane_343_gpwe_lpwe_cpwe_cpwe.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/reconstructions/rec_1dcsc.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/reconstructions/nmse_distance_monopole.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/sfrtest/particle_velocity_gpwe_monoplane.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/sfrtest/particle_velocity_cpwe_monoplane.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/sfrtest/particle_velocity_lpwe_monoplane.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/1dpartitioning.pdf ./fig/
	@cp $(DTUDIR)/rat/figures/mc/csc_paper_* ./fig/

clean-post-build:
	@rm *.{aux,snm,toc,nav,ps,log,out,dvi,bbl,bcf,blg,run.xml,dpth,md5,auxlock,synctex.gz} 2> /dev/null
	@rm $(OUTPUT)/*.{dpth,md5,auxlock,log} 2> /dev/null

.PHONY: clean
clean:
	@rm *.{ps,log,out,dvi,bbl,bcf,blg,run.xml,dpth,md5,auxlock,synctex.gz} 2> /dev/null 2> /dev/null
	@rm $(OUTPUT)/* 2> /dev/null

clean_all:
	@rm *.{pdf,ps,log,aux,out,dvi,bbl,bcf,blg,run.xmldpth,md5,auxlock,synctex.gz} 2> /dev/null
	@rm $(OUTPUT)/* 2> /dev/null
